Efficient Simulation of Singularly Perturbed Systems Using a Stabilized Multirate Explicit Scheme

Singularly perturbed systems (SPSs) are prevalent in engineering applications, where numerically solving their initial value problems (IVPs) is challenging due to stiffness arising from multiple time scales. Classical explicit methods require impractically small time steps for stability, while implicit methods developed for SPSs are computationally intensive and less efficient for strongly nonlinear systems. This paper introduces a Stabilized Multirate Explicit Scheme (SMES) that stabilizes classical explicit methods without the need for small time steps or implicit formulations. By employing a multirate approach with variable time steps, SMES allows the fast dynamics to rapidly converge to their equilibrium manifold while slow dynamics evolve with larger steps. Analysis shows that SMES achieves numerical stability with significantly reduced computational effort and controlled error. Its effectiveness is illustrated with a numerical example.

==> handnote.tex <==
\section*{Appendix}

However, when applying explicit methods like the Forward Euler method to singularly perturbed systems, the choice of time step becomes critical due to the stiffness introduced by the small parameter $\varepsilon$. The fast dynamics necessitate exceedingly small time steps to maintain numerical stability, which can render simulations computationally impractical. To systematically analyze this issue and understand the limitations of explicit methods, we employ simplified test equations that capture the essential features of singularly perturbed systems. 

Using test equations is a well-established practice in numerical analysis for investigating the stability and convergence properties of numerical methods applied to stiff systems \cite{Hairer1996SolvingODEs, Butcher2016NumericalMethods}. These simplified models allow for analytical tractability while retaining the key characteristics that influence the behavior of numerical schemes. By focusing on test equations, we can derive explicit stability conditions and gain valuable insights into how the time step size affects the performance of methods like Forward Euler. This approach not only highlights the challenges posed by stiffness but also guides the development of more efficient numerical algorithms tailored to singularly perturbed systems. 



In this report, we choose to use a singularly perturbed autonomous CT linear model as the test system, which has the following form:
\begin{equation}\label{eq:testeq}
\begin{aligned}
    \dot{x} &= a x_k + b z_k, \\
    \epsilon \dot{z} &= c x_k + d z_k,
\end{aligned}
\end{equation}
where the state-variable $x$ and $z$ are scalar for convenience of expression. The test system is assumed to be asymptotically stable, namely that:
\begin{equation}
    \begin{aligned}
        \lambda_{1, 2} &= \frac{1}{2\epsilon}(\epsilon a + d \pm \sqrt{(\epsilon a - d)^2 + 4\epsilon bc}) < 0. 
    \end{aligned}
\end{equation}
For the fast dynamics to be underdamped, the system coefficients satisfy the following:
\begin{equation*}
    (\epsilon a - d)^2 + 4\epsilon bc > 0.
\end{equation*}

Applying the Forward Euler approximation with step size $\Delta$ to the test system in Eq. \eqref{eq:testeq} yields the following discrete-time (DT) SS model:
\begin{equation}\label{eq:forwardeuler}
\begin{aligned}
    x_{k+1} &=x_k + \Delta a x_k + \Delta b z_k, \\
    z_{k+1} &=z_k + \frac{\Delta c}{\epsilon} x_k +  \frac{\Delta d}{\epsilon} z_k,
\end{aligned}
\end{equation}
where $k$ denotes the time step index, and $x_k$, $z_k$ denote the states at time $t = \Delta k$. Due to the introduction of the singular perturbation, the discretized model also possesses some very fast dynamics (with time constants of order $O(\epsilon)$), so the approximate model \eqref{eq:forwardeuler} may suffer from numerical instability unless $\Delta = O(\epsilon)$, since for numerical stability of the forward Euler method it is necessary and sufficient that $|1 + \lambda \Delta| < 1$ for every eigenvalue $\lambda$ of the CT test system. In particular, this condition, in the underdamped case, is the following:
\begin{equation}
    \begin{aligned}
        &\ \ |1 + \frac{\Delta}{2\epsilon}(\epsilon a + d \pm \sqrt{(\epsilon a - d)^2 + 4\epsilon bc})| < 1\\
        &\Leftrightarrow (1 + \frac{\Delta a}{2} + \frac{\Delta d}{2\epsilon})^2 + \frac{\Delta^2}{4\epsilon^2} (\epsilon a - d)^2 + \frac{\Delta^2}{\epsilon} bc < 1\\
        &\Leftrightarrow (\frac{a}{2} + \frac{bc}{\epsilon} + \frac{d}{2\epsilon^2})\Delta^2 + (a + \frac{d}{\epsilon})\Delta < 0\\
        &\Leftrightarrow \Delta < \frac{2\epsilon^2a + 2\epsilon d}{\epsilon^2a + 2\epsilon bc + d} = O(\epsilon)
    \end{aligned}
\end{equation}

% For a fixed small parameter $\epsilon$ in a specific system, the Forward Euler method gives the following discrete-time (DT) SS model:
% \begin{equation}\label{eq:forwardeuler}
% \begin{aligned}
%     x_{k+1} &= x_k + h f(x_k, z_k, u_k), \\
%     z_{k+1} &= z_k + \frac{h}{\epsilon} g(x_k, z_k, u_k),
% \end{aligned}
% \end{equation}
% where $h$ is the step size, $k$ denotes the time step index, and $x_k$, $z_k$ denote the states at time $t = hk$. 

% Considering only the fast dynamics, we can linearize the equation for $z_{k+1}$ as: 
% \begin{equation}\label{eq:linearz}
%     z_{k+1} = z_k + \frac{h}{\epsilon} J^k_z z_k + \frac{h}{\epsilon} J^k_x x_k + \frac{h}{\epsilon} J^k_u u_k + \frac{h}{\epsilon}\text{h.o.t.} , 
% \end{equation}
% where 
% $$
% \begin{aligned}
%     J^k_x &= \frac{\partial g(x, z, u)}{\partial x} \mid_{x = x_k, z = z_k, u = u_k},\\
%     J^k_z &= \frac{\partial g(x, z, u)}{\partial z} \mid_{x = x_k, z = z_k, u = u_k},\\
%     J^k_u &= \frac{\partial g(x, z, u)}{\partial u} \mid_{x = x_k, z = z_k, u = u_k}.
% \end{aligned}
% $$

% Note that the high-order terms (h.o.t.) in Eq. \eqref{eq:linearz} are introduced by the local linearization of the function $g(\cdot)$ which usually satisfies $|\text{h.o.t.}| \le O(\epsilon)$. Therefore, the equation for $z+{k+1}$ can be approximate by the following:
% \begin{equation}\label{eq:linearapprox}
%     z_{k+1} \approx z_k + \frac{h}{\epsilon} J^k_z z_k + \frac{h}{\epsilon} J^k_x x_k + \frac{h}{\epsilon} J^k_u u_k, 
% \end{equation}

% The stability of the discretized equation in Eq. \eqref{eq:linearz} requires the eigenvalues of the matrix $( I + \frac{h}{\varepsilon} J^k_z )$ to lie within the unit circle. This condition can be expressed as:

% \begin{equation}
%     \left| I + \frac{h}{\varepsilon} \lambda_{J^k_z} \right| \leq I,
% \end{equation}
% where $\lambda_{J^k_z}$ is an eigenvalue of the matrix $J^k_z$. By expanding the above inequality, we get:
% \begin{equation*}
%     -2 I \leq \frac{h}{\varepsilon} \lambda_{J^k_z} \leq 0,
% \end{equation*}
% which implies that:
% \begin{equation}
%     h \leq \frac{2 \varepsilon}{|\lambda^{max}_{J^k_z}|} = O({\epsilon}),
% \end{equation}
% where $|\lambda^{max}_{J^k_z}|$ is the magnitude of the largest eigenvalue of the matrix $J^k_z$.

Thus, the step size $\Delta$ is constrained by the smallest time scale, which is governed by the fast dynamics. This implies that as $\varepsilon \rightarrow 0$, the step size $\Delta$ must also decrease significantly. This results in
a large number of time steps to cover the desired simulation time $T$, i.e., $\frac{T}{\epsilon} = O(\frac{1}{\epsilon})$ times the evaluations of functions, leading to an increased computational cost and simulation time. 

Given this limitation, this study aims to develop a more efficient method that handles the singular perturbation introduced by the fast dynamics without resorting to prohibitively small step sizes. In the following section, an efficient simulation scheme is introduced which allows for faster and stable simulations of singularly perturbed systems using explicit methods. 

% First, we consider the linear approximation of the discretized fast subsystem with the short step $\Delta\epsilon$ as follows: 
% \begin{equation}
%     z_{k+1} \approx z_k + \Delta J^k_z z_k + \Delta J^k_x x_k + \Delta J^k_u u_k, 
% \end{equation}
% where the system matrix is $(I + \Delta J^k_z)$ and $\Delta \leq \frac{2}{|\lambda_{J^k_z}^{max}|}$. As in Algorithm \ref{alg:proposed_scheme}, the short step $\Delta\epsilon$ is taken $n$ times where $n = 1,\dots,N$. Therefore, the general discretized fast subsystem has the following form:
% \begin{equation}
%     z_{k+n} \approx z_{k+n-1} + \Delta J^{k+n-1}_z z_{k+n-1} + \Delta J^{k+n-1}_x x_{k+n-1} + \Delta J^{k+n-1}_u u_{k+n-1}, 
% \end{equation}
% where for every system matrix $(I + \Delta J^{k+n-1}_z)$ we should have $\Delta \leq \frac{2}{|\lambda_{J^{k+n-1}_z}^{max}|}$. Assume that for the upper bound on the magnitude of $|\lambda_{J^{k+n}_z}^{max}|$ is defined by $｜\tilde{\lambda}｜$, then the fast subsystem is guaranteed to evolve within the boundary system within $N$ short steps as follows:
% \begin{equation}
%     z_{k+N} = (I + \Delta \tilde{\lambda})^N z_k,
% \end{equation}
% where the necessary and sufficient condition for the boundary system to be stable is that $\Delta \leq \frac{2}{|\tilde{\lambda}|}$.


Combined with the one large step of length $(1 - N\epsilon)$ taken after the $N$ small time steps, the boundary system of DT fast subsystem is as follows:
\begin{equation}
    \ve{z}(t + \Delta) \approx \underbrace{\left( \ve{I} + \frac{\Delta}{\epsilon} (1 - N \epsilon) \tilde{\lambda} \right) \left( \ve{I} + \Delta \tilde{\lambda} \right)^N}_{=: \ve{A}_\Delta} \ve{z}(t).
\end{equation}

The discretized fast subsystem is guaranteed stable if the eigenvalues of $\ve{A}_\Delta$ are smaller than one in magnitude. Thus, for stability, it is sufficient that
\begin{align} \label{eq:stability_condition}
|1 + \Delta(1 - N \epsilon) \frac{\tilde{\lambda}}{\epsilon}| |1 + \Delta \tilde{\lambda}|^N < 1.
\end{align}

Assume that $0 < \epsilon \ll 1$, and $\tilde{\lambda} = O(1)$. Condition~\eqref{eq:stability_condition} is approximately equivalent (for small $\epsilon$) to
\begin{align*}
N \geq - \frac{\ln |1 + \Delta \frac{\tilde{\lambda}}{\epsilon} - N \Delta \tilde{\lambda}|}{\ln |1 + \Delta \tilde{\lambda}|}.
\end{align*}

For very small $\epsilon$, while keeping $N$ and $\Delta$ fixed, we notice that $\ln |1 + \Delta \frac{\tilde{\lambda}}{\epsilon} - N \Delta \tilde{\lambda}| > 0$, so for \eqref{eq:stability_condition} to be satisfied we first need that $\ln |1 + \Delta \tilde{\lambda}| < 0$, \ie, $|1 + \Delta \tilde{\lambda}| < 1$. Under this assumption, and considering that $\epsilon \ll 1$, while keeping $\Delta$ fixed and assuming $N$ is smaller than $1/\epsilon$, we obtain the approximate condition

\begin{align} \label{eq:approx_stab_condition_fast}
N \geq - \frac{\ln (\Delta |\tilde{\lambda}| / \epsilon)}{\ln |1 + \Delta \tilde{\lambda}|} = O(\ln(1 / \epsilon)).
\end{align}

This expression confirms that the assumption $N \ll 1/\epsilon$ can be satisfied. Notice that while the condition on $N$ is not independent of $\epsilon$, its dependence is very mild due to the logarithm in \eqref{eq:approx_stab_condition_fast}.

% It is interesting to note that, if one could choose $\Delta$ such that $1 + \Delta \tilde{\lambda} \approx 0$ (while ensuring that $|1 + \Delta \lambda| < 1$ for all slow poles), then the number of iterations $N$ can be reduced considerably. This is because the base in the second factor in \eqref{eq:stability_condition} becomes approximately zero (\ie, the forward Euler discretization of the fast subsystem has a \emph{dead-beat} response).

In terms of computational effort, the variable-step Forward Euler scheme requires
\begin{align*}
(N + 1) \frac{T}{\Delta}
= O\left( - \frac{\ln (\Delta |\tilde{\lambda}| / \epsilon)}{\ln |1 + \Delta \tilde{\lambda}|} \frac{T}{\Delta} \right)
=  O(T \tilde{\lambda} \ln [1 / \epsilon])
\end{align*}
function evaluations in order to simulate the model for a time duration of $T$ with the stability guarantee, since $\Delta = O(1/\tilde{\lambda})$. Notice that this number depends only mildly on the small variable $\epsilon$. 

